iSign: A Benchmark for Indian Sign Language Processing

Indian Sign Language has limited resources for developing machine learning and data-driven approaches for automated language processing. Though text/audio-based language processing techniques have shown colossal research interest and tremendous improvements in the last few years, Sign Languages still need to catch up due to the need for more resources. To bridge this gap, in this work, we propose iSign: a benchmark for Indian Sign Language (ISL) Processing. We make three primary contributions to this work. First, we release one of the largest ISL-English datasets with more than 118K video-sentence/phrase pairs. To the best of our knowledge, it is the largest sign language dataset available for ISL. Second, we propose multiple NLP-specific tasks (including SignVideo2Text, SignPose2Text, Text2Pose, Word Prediction, and Sign Semantics) and benchmark them with the baseline models for easier access to the research community. Third, we provide detailed insights into the proposed benchmarks with a few linguistic insights into the workings of ISL. We streamline the evaluation of Sign Language processing, addressing the gaps in the NLP research community for Sign Languages. We release the dataset, tasks, and models via the following website: https://exploration-lab.github.io/iSign/

==> sections/challenges.tex <==
% \vspace{-3mm}
\section{Technical Limitations and Challenges} \label{sec:limitations}
% \vspace{-3mm}
The large number of ISL-English sentence pairs in the initial version of the dataset makes it challenging to validate. Though we provide a small-scale validation with an ISL instructor's help, the entire corpus's validation is tedious, and it is infeasible to look into minute aspects of ISL-English translations in an initial version. In the future, we plan to extend the validation task and add a gold translation set with multiple references provided for a set of 5K ISL sentences. For an initial version of the benchmark, it is imperative to consider some possible technical constraints in the dataset. We believe addressing these constraints is a long-term goal, and mentioning them in detail will open up various directions for future work on analyzing and improving the benchmark.

\noindent\textbf{Alignment in ISL-English Pairs:} As the \benchmarkName\ translation dataset consists of sentence-level videos clipped from a longer video using multiple strategies, pauses in the available audio signal for ISLRTC videos, frame pattern heuristics for DEF videos, and available English caption timestamps for ISH videos, there are multiple ways in which the alignment between ISL signing sentence and corresponding English Sentence is disrupted. For example, in ISLRTC videos, though the audio in the background is aligned with the corresponding signs in the video, it could happen in a few cases that the audio was fast compared to the corresponding sign representation and may miss a few words at the beginning or the end of the sentence. Similarly, for ISH videos, the timestamps in the captions might be delayed or fast in a few cases.

\textbf{\textbf{Co-referencing in ISL:}} As mentioned in Section \ref{sec:linguistics}, ISL linguistics involves assigning various short signs for names, places, etc., with various spatial reference points to refer to places defined for a specific conversation, making the context an essential feature for a complete translation of the content. As the translation dataset in \benchmarkName\ was created by segmenting a longer video into shorter segments representing a sentence, there is a high possibility that the names in the sentences are introduced in different sentences and assigned a short sign, which may be difficult to refer to in the later sentences. We consider this a major limitation of the created ISL-English pair dataset, as translating the same names would be difficult without a given reference to the created short sign or allocated space, and the independently made translations would result in a lower score in evaluation metrics like BLEU. One way of addressing this challenge would be to perform a task similar to NER on the ISL videos. However, the unavailability of resources and the scarcity of certified signers make ISL video annotation more challenging. 

\noindent\textbf{Presence of Role Shifts:} As a major portion of the created dataset comes from educational content created by ISLRTC, a lot of material contains stories with fictional characters. In stories, there exists a high possibility of Role Shifts when producing sentences spoken by a character. A similar example in spoken storytelling would be the change in voice to articulate a character's voice, for example, the use of a squeaky voice for enacting the sentences of a small mouse. Since these Role Shifts are produced via non-manual markers, they would result in slight gesture variations for the same sentence, making the translated sentence more challenging to predict.

% \noindent\textbf{Poor Performance of Existing Baseline Models:} As observed earlier, the current baseline models for several tasks show poor performance, pointing towards the development of more sign-language-specific neural architectures in the future. The machine translation baselines, which show SOTA performance on datasets like Phoenix-2014T and CSL-Daily, do not perform well for the created dataset. Most existing approaches for sign language translation \cite{phoenix_dataset, info13050220, De_Coster_2021_AT4SSL, chen2022two-stream} depend on intermediate gloss labels for translations. As glosses are aligned to video segments, they provide fine one-to-one mapping that facilitates supervised learning in learning effective video representations. Previous work has reported a drop of about $10.0$ in BLEU-4 scores without gloss labels \cite{phoenix_dataset}. However, considering the annotation cost of gloss-level annotations, it becomes imperative to consider gloss-free sign language translation approaches. Moreover, the gloss mapping in continuous sign language might remove the grammatical aspects from the sign language. The presence of gloss labels for sign sentences in a dataset helps translation systems to work at a granular level of sign translation. However, generating gloss annotations for a signed sentence is an additional challenge due to the scarcity of certified signers. The large number of samples present in the created dataset makes the gloss-level annotation infeasible. There are a few recent works on Sign language translation \citet{Voskou2021StochasticTN, yin-read-2020-better}, which try to remove the requirement for a glossing sequence for training and propose a transformer-based architecture for end-to-end translations. Moreover, the noteworthy point is that the dataset size of \benchmarkName\  differs from Phoenix-2014T and CSL-Daily by a significant margin (138k vs. 8.2k, 20.6k), making \benchmarkName\  more diverse with high variance in gestures/signs, which might also be one of the reasons for poor performance.

% \noindent\textbf{Evaluation Metric for Sign Generation:} In the current version of the \benchmarkName\  benchmark, we use the Dynamic Time Warping (DTW) algorithm to evaluate the quality of generated sign pose key points. The DTW algorithm has limitations in dealing with significant variations in motion between the generated and ground truth sequences. Moreover, the DTW may not be suitable for measuring the quality of generated sign language. While designing the evaluation metrics, it is essential to consider sign language's linguistic aspects and ensure they correlate strongly with human evaluation. 
% Future work can be focused on exploring gesture generation works \citep{gesturereview} that can better capture the nuances of sign language. 

% \section{Future Directions}

% \begin{enumerate}
%     \item \textbf{Suitable Evaluation metrics}: The Dynamic Time Warping (DTW) algorithm, used to align the generated pose sequences with the ground truth, has limitations in dealing with large variations in motion between the generated and ground truth sequences. The back translation models employed for evaluating the generation models themselves are insufficient. While designing the evaluation metrics, it is essential to consider the linguistic aspects of sign language and ensure they possess a strong correlation with human evaluation. Future work can be focused on exploring gesture generation works \cite{gesturereview} that can better capture the nuances of sign language. 

%     % \item Additionally, sign language is a complex and dynamic language that involves not only hand movements but also facial expressions, body language, and non-manual markers. Our model focuses on generating hand and facial movements but does not address the other non-manual components. It is crucial to explore the inclusion of non-manual markers, such as body language and gaze direction, in the generation process to improve the naturalness and effectiveness of sign language communication.

%     \item \textbf{Variations in Signer Style}: Sign language is highly dependent on the signer's individual style and preferences, which can significantly affect the performance of the models. In future work, it is necessary to explore the impact of varying signer styles on the performance of the sign language processing models.
% \end{enumerate}


% \AJ{leaderboard addition in future, can mention in conclusion as well}


==> sections/checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
%The checklist follows the references.  Please read the checklist guidelines carefully for information on how to answer these questions.  For each question, change the default \answerTODO{} to \answerYes{},\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf justification to your answer}, either by referencing the appropriate section of your paper or providing a brief inline description.  For example:

% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
   \textcolor{blue}{\textbf{Yes}}
  \item Did you describe the limitations of your work?
   \textcolor{blue}{\textbf{Yes, section 7}}
  \item Did you discuss any potential negative societal impacts of your work?
    \textcolor{blue}{\textbf{NA}}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \textcolor{blue}{\textbf{Yes}}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \textcolor{blue}{\textbf{NA}}
	\item Did you include complete proofs of all theoretical results?
    \textcolor{blue}{\textbf{NA}}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \textcolor{blue}{\textbf{Yes, in appendix}}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \textcolor{blue}{\textbf{Yes, in appendix}}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \textcolor{blue}{\textbf{Yes, in appendix}}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \textcolor{blue}{\textbf{Yes, in appendix}}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \textcolor{blue}{\textbf{Yes}}
  \item Did you mention the license of the assets?
    \textcolor{blue}{\textbf{Yes}}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \textcolor{blue}{\textbf{Yes, in github link}}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \textcolor{blue}{\textbf{Yes}}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \textcolor{blue}{\textbf{NA}}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \textcolor{blue}{\textbf{NA}}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \textcolor{blue}{\textbf{NA}}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \textcolor{blue}{\textbf{NA}}
\end{enumerate}

\end{enumerate}
